Phase Transition in Extended Thermodynamics Triggers Sub-shocks

Extended thermodynamics commonly uses polynomial moments to model non-equilibrium transportation, but faces a crisis due to sub-shocks, which are anomalous discontinuities in gas properties when predicting shock waves. The cause of sub-shocks is still unclear, challenging the validity of extended thermodynamics. This paper reveals, for the first time, that sub-shocks arise from intrinsic limitations of polynomials leading to a discontinuous phase transition. Therefore extended thermodynamics necessitates alternative moments beyond polynomials to avoid sub-shocks.

==> deleted.tex <==
Extended thermodynamics of moments generalizes classical thermodynamics to describe non-equilibrium gas behavior, such as shock waves. However, it faces a notorious issue when calculating gas shock waves: sub-shocks. Sub-shocks are non-realistic discontinuities in the shock wave profile predicted by extended thermodynamics whose physical formation mechanism remains unclear. This paper shows that sub-shock is triggered by phase transition, a discontinuous change from single-peaked to dual-peaked molecular distributions at the front of the shock wave. This change is discontinuous because polynomial moments used in extended thermodynamics cannot describe the change-in-peak continuously. Therefore extended thermodynamics needs more general moments other than polynomial moments to eliminate the sub-shock issue.


Non-equilibrium processes in gases, including shock waves, are crucial for understanding various phenomena in fluid dynamics, aerospace engineering, and astrophysics. Traditional approaches to modeling these processes, such as the Navier-Stokes-Fourier (NSF) equations, often fail to capture non-equilibrium behavior accurately. Extended thermodynamics has emerged as a promising framework to address these limitations by incorporating additional variables and equations to describe higher-order moments. These higher-order moments provide a more detailed representation of the behavior of a gas under non-equilibrium conditions, capturing transport properties of gases such as stress and heat flux hence describing non-equilibrium processes more accurately.


To analyze the sub-shocks, we also need to specify the polynomial statistics $\phi_n(\mathbf{u})$ used in the exponential family model. Specifying the polynomial statistics $\phi_n(\mathbf{u})$ requires prior knowledge about the shock wave. Considering a normal shock wave propagating along the x direction with no tangent flow velocity, we can make two key assumptions: Firstly, we assume that the local maxima of $\log f(\mathbf{r}, \mathbf{u}, t)$ only occur at $u_y = u_z = 0$ in order to ensure a stable shock profile. This assumption implies that the local maxima of $\log f(\mathbf{r}, \mathbf{u}, t)$ is fully determined by a polynomial in $u_x$. Secondly, we assume that across the shock wave, the distribution function $f(\mathbf{r}, \mathbf{u}, t)$ has up to two peaks. This is a well-known prior used by the Mott-Smith model for normal shock waves, which implies that $\log f(\mathbf{r}, \mathbf{u}, t)$ should have three extreme points consisting of two maxima and one minimum. These assumptions suggest that we should choose polynomial moments systems consisting of 4th order polynomials, which is the 35 moment system. For 1D flow like normal shock wave, the 35 moment system of polynomial statistics $\phi_n(\mathbf{u})$ can be defined as follows:
\begin{equation}
\label{Sufficient 35}
\begin{split}
\{\phi_i(\bold{u})\} &= \{1, u_x, u_x^2, u_x^3, u_x^4, u_r^2, u_r^4, u_x u_r^2, u_x^2 u_r^2\}
\end{split}
\end{equation}
in which $u_r = \sqrt{u_y^2 + u_z^2}$. 


The 35-moment system permits two local maxima but is unable to describe them independently. For each local maximum $u_{1,2}^*$, the polynomial derivative $\log f'(u_{1,2}^*)$ vanishes, while the extreme value $\log f_{1,2} = \log f(u_{1,2}^*)$ and the curvature $t_{1,2} = -\log f''(u_{1,2}^*)$ at these points determine their contributions to the saddle point approximation. Consequently, each local maximum demands three degrees of freedom, corresponding to extreme value, derivative, and curvature, for complete specification. However, the 35-moment system's polynomial $\log f(u_x)$ possesses only five free $\lambda$ parameters, which are insufficient for independently describing the two local maxima that require at least six degrees of freedom. As a result, the two local maxima are entwined, with their extreme values, locations, and curvatures interconnected by the equation
\begin{equation}
\log f_2 - \log f_1=\frac{1}{12} (t_2-t_1) (u_{2}^*-u_{1}^*)^2.
\end{equation}
This interconnection constrains the relative values and locations of the two local maxima, thus preventing a smooth distribution transition from single-peak to dual-peak profiles, leading to a discontinuous phase change that induces sub-shocks.

However, a significant challenge in extended thermodynamics is the presence of unrealistic sub-shocks in its predicted shock wave profiles. Sub-shocks are discontinuous changes in gas properties that emerge within the shock wave profiles and contradict experimental observations, indicating potential insufficiency in the current formulation of extended thermodynamics. The traditional approach to analyzing sub-shocks in extended thermodynamics is characteristic speeds of the moment equations. The characteristic speeds, denoted as $v_n$, are given by the eigenvalues of the matrix formed by the coefficients of the spatial derivatives in the moment equations. Mathematically, this can be represented as $A_{m n} \equiv \frac{\partial \mathbf{F}_{n,x}}{\partial M_m}$.
The characteristic speeds are then obtained as $v_n = \text{eig}(\mathbf{A})$. Sub-shocks may appear when the shock velocity meets any of the characteristic speeds, indicating potential phase transitions in the gas. However, such analysis is local and does not provide detailed information about the distribution function, making it difficult to identify the cause of sub-shocks.


In addition, we define the partition function $Z(\lambda_0, \cdots, \lambda_n)$ of the exponential family model as 
\begin{equation}
    Z(\lambda_0, \cdots, \lambda_n) =  \int \exp{\left(\sum_{n = 0}^{N} \lambda_n(\mathbf{r}, t) \cdot \phi_n(\mathbf{u}) \right) } d\mathbf{u},
\end{equation}
from which we could compute moments $M_n(\mathbf{r}, t)$ by taking derivatives w.r.t $\lambda_n$
\begin{equation}
  M_n(\mathbf{r}, t) = \frac{\partial Z}{\partial \lambda_n},
\end{equation}

In this paper, we adopt the BGK collision model to describe the collision process. The flux and source terms in the moment equations for the BGK model can be defined as:
\begin{equation}
\mathbf{F}_n(\mathbf{r}, t) = \int \mathbf{u} \phi_n(\mathbf{u})  f(\mathbf{r}, \mathbf{u}, t) d\mathbf{u},
\end{equation}
\begin{equation}
\mathbf{S}_n(\mathbf{r}, t) = \frac{M_n^{eq}(\mathbf{r}, t) - M_n(\mathbf{r}, t)}{\tau},
\end{equation}
where $M_n^{eq}(\mathbf{r}, t)$ is the equilibrium value of the $n$-th moment, and $\tau$ represents the relaxation time, which characterizes the time scale of the collision process. The relaxation time is determined by various factors, such as gas properties, temperature, and pressure. 

The moment equations form the core of extended thermodynamics. They are conservation laws that govern the time evolution of moments $M_n$ and Lagrangian multipliers $\lambda_n$. They can be derived by substituting the exponential family model into the Boltzmann equation. These equations can be written in a general form:
\begin{equation}
\partial_t M_n + \sum_{\alpha \in \{x,y,z\}} \partial_\alpha F_{n,\alpha} = \mathbf{S}_n,
\end{equation}
where $F_{n,\alpha}$ represents the flux of the $n$-th moment in the $\alpha$ direction, and $\mathbf{S}_n$ is a source term that accounts for various physical processes, such as collisions, radiative transport, or chemical reactions. In practice, we solve these moment equations numerically using the Lax-Friedrich method. The detailed formulation of flux and source terms, boundary conditions, and numerical schemes are given in \cite{zheng2023stabilizing}. The shock wave predicted by these moment equations matches the reference DSMC results nicely despite a small sub-shock appearing at the front of the shock wave.


In order to examine the sub-shocks, we must first define the polynomial statistics $\phi_n(\mathbf{u})$ utilized in the exponential family model. Specifying these statistics calls for prior knowledge about the shock wave. For a normal shock wave propagating along the x-axis without tangent flow velocity, we make two main assumptions. First, we assume that the local maxima of $\log f(\mathbf{r}, \mathbf{u}, t)$ only occur at $u_y = u_z = 0$, ensuring a stable shock profile. This assumption means that the local maxima of $\log f(\mathbf{r}, \mathbf{u}, t)$ is entirely determined by a polynomial in $u_x$. Second, we assume that the distribution function $f(\mathbf{r}, \mathbf{u}, t)$ has a maximum of two peaks across the shock wave. This prior is commonly used in the Mott-Smith model for normal shock waves and implies that $\log f(\mathbf{r}, \mathbf{u}, t)$ should have three extreme points, consisting of two maxima and one minimum.

These assumptions lead us to choose a 35 moment system of polynomial statistics $\phi_n(\mathbf{u})$, consisting of 4th order polynomials that admits two maxima, as shown in Equation (\ref{Sufficient 35}). For one-dimensional flow, such as normal shock waves, the 35 moment system can be defined as follows:

\begin{equation}
\label{Sufficient 35}
\begin{split}
\{\phi_i(\bold{u})\} &= \{1, u_x, u_x^2, u_x^3, u_x^4, u_r^2, u_r^4, u_x u_r^2, u_x^2 u_r^2\},
\end{split}
\end{equation}
where $u_r = \sqrt{u_y^2 + u_z^2}$. In this moment system, the local maxima of the distribution function take the form $\mathbf{u}^* = \{u_x^*,0,0\}$, with $u_x^*$ being the local maxima of the polynomial:

\begin{equation}
\begin{split}
\log f(u_x) &= \lambda_0 + \lambda_1 u_x + \lambda_2 u_x^2 + \lambda_3 u_x^3 + \lambda_4 u_x^4
\end{split}
\end{equation}
which admits at most two maximum separated by a minimum.



The behavior of the distribution function near the sub-shock can be further analyzed by investigating the stress in the shock wave. To achieve this, we employ the saddle point approximation, focusing on the stress dependence on the position $u_2^*$ and the curvature $t_2$ of the second local maximum. The stress of the shock wave, $\sigma_{xx}$, can be approximated as:
\begin{equation} \label{sigma equation}
\sigma_{xx} \propto t_2^{-3/2}(u_1^*-u_2^*)^2 e^{\frac{1}{12} (t_2-t_1) (u_1^*-u_2^*)^2},
\end{equation}
This equation allows us to closely examine the changes in the second local maximum $u_2^*$. Near the downstream of the sub-shock, $u_2^*$ varies rapidly without significant changes in $u_1^*$, $t_1$, and the stress $\sigma_{xx}$. Consequently, the local maximum $u_2^*$ and its curvature $t_2$ lie on the contour line of Equation \eqref{sigma equation}, keeping $\sigma_{xx}$ constant. Specifically, as $u_2^*$ increases, the curvature $t_2$ decreases, indicating that the second local maximum becomes wider as we move from the sub-shock towards the downstream direction. This observation confirms that the sub-shock corresponds to the phase transition (1) in Figure 1, where a narrow second peak appears and gradually widens, transitioning from a single-peak to a dual-peak profile.

(Discontinuous emergence and smooth disappearance) Two phase diagrams for a Mach 4 normal shock wave, computed by the extended thermodynamics using the 35 polynomial moment system. Diagram 
